Introduction to Online Convex Optimization

This manuscript portrays optimization as a process. In many practical applications the environment is so complex that it is infeasible to lay out a comprehensive theoretical model and use classical algorithmic theory and mathematical optimization. It is necessary as well as beneficial to take a robust approach, by applying an optimization method that learns as one goes along, learning from experience as more aspects of the problem are observed. This view of optimization as a process has become prominent in varied fields and has led to some spectacular success in modeling and systems that are now part of our daily lives.

==> abstract.tex <==
\chapter*{Abstract}

This manuscript portrays  {\it optimization as a process}.  In many practical applications the environment is so complex that it is infeasible  to lay out a comprehensive theoretical model and use classical algorithmic theory and mathematical optimization. It is necessary as well as beneficial to take a robust approach, by applying an optimization method that learns as one goes along, learning from experience as more aspects of the problem are observed. 
This view  of optimization as a process has become prominent in varied fields and has led to some spectacular success in modeling and systems that are now part of our daily lives. 

